A Hybrid Cable-Driven Robot for Non-Destructive Leafy Plant Monitoring and Mass Estimation using Structure from Motion

We propose a novel hybrid cable-based robot with manipulator and camera for high-accuracy, medium-throughput plant monitoring in a vertical hydroponic farm and, as an example application, demonstrate non-destructive plant mass estimation. Plant monitoring with high temporal and spatial resolution is important to both farmers and researchers to detect anomalies and develop predictive models for plant growth. The availability of high-quality, off-the-shelf structure-from-motion (SfM) and photogrammetry packages has enabled a vibrant community of roboticists to apply computer vision for non-destructive plant monitoring. While existing approaches tend to focus on either high-throughput (e.g. satellite, unmanned aerial vehicle (UAV), vehicle-mounted, conveyor-belt imagery) or high-accuracy/robustness to occlusions (e.g. turn-table scanner or robot arm), we propose a middle-ground that achieves high accuracy with a medium-throughput, highly automated robot. Our design pairs the workspace scalability of a cable-driven parallel robot (CDPR) with the dexterity of a 4 degree-of-freedom (DoF) robot arm to autonomously image many plants from a variety of viewpoints. We describe our robot design and demonstrate it experimentally by collecting daily photographs of 54 plants from 64 viewpoints each. We show that our approach can produce scientifically useful measurements, operate fully autonomously after initial calibration, and produce better reconstructions and plant property estimates than those of over-canopy methods (e.g. UAV). As example applications, we show that our system can successfully estimate plant mass with a Mean Absolute Error (MAE) of 0.586g and, when used to perform hypothesis testing on the relationship between mass and age, produces p-values comparable to ground-truth data (p=0.0020 and p=0.0016, respectively).

==> 5_discussion.tex <==
Our dataset evidences the efficacy and utility of our robot data collection platform.  The speed and consistency with which photos are taken allows for higher throughput and quality data collection.  We can compare the cable robot against 2 other baseline methods tested: (1) single top-down images and (2) an automated robot arm without cable robot.

% Fig. \ref{fig:dataset_iphone} depicts the results from baseline 1: single top-down images.  Although this has a low human labor requirement, the maximum information that can be extracted from this data alone is limited.  Prior work analyzing this dataset exhibits poor generalization to different nutrient schedules, with excess of 100\% error for certain nutrient schedules, as shown in Fig. \ref{fig:results_iphone}.
% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\linewidth]{figs/iphone.jpeg}
%   \caption{Photos from baseline 1 of top-down photos from an iPhone camera (prior work by Andrew Sharkey).  Only a single photo per plant was taken, limiting the comprehensiveness and predictive power of the data.}
%   \label{fig:dataset_iphone}
% \end{figure}
% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\linewidth]{figs/iphone_regression-eps-converted-to.pdf}
%   \caption{Regression result using top-down photos from baseline 1 (prior work by Sushmita Warrier).}
%   \label{fig:results_iphone}
% \end{figure}

Fig. \ref{fig:dataset_arm} depicts the results from baseline 2: photos taken by a robot arm but without the cable robot.  Because the robot arm alone can only reach a single plant, a human is required to manually place the robot at each plant which not only increases human labor cost, but also introduces additional variability in the data due to imprecise robot placement.  Both issues eliminate the possibility of this approach for high-throughput phenotyping in the current laboratory environment.


